Photo style transfer with consistency losses

We address the problem of style transfer between two photos and propose a new way to preserve photorealism. Using the single pair of photos available as input, we train a pair of deep convolution networks (convnets), each of which transfers the style of one photo to the other. To enforce photorealism, we introduce a content preserving mechanism by combining a cycle-consistency loss with a self-consistency loss. Experimental results show that this method does not suffer from typical artifacts observed in methods working in the same settings. We then further analyze some properties of these trained convnets. First, we notice that they can be used to stylize other unseen images with same known style. Second, we show that retraining only a small subset of the network parameters can be sufficient to adapt these convnets to new styles.

==> fig/figure_reapply_details.tex <==
\begin{figure*}
\begin{center}
\captionsetup[subfigure]{font=scriptsize}
%
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in4.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar4.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in31.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar31.png}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in4.png}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar4.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_4.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar4_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_4_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_7.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar7_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_7_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_10.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar10_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_10_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_19.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar19_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in31.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_19_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar31.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply/tar31_random/test_post_31.PNG}
\end{subfigure}
\hspace{0.086\linewidth}

\end{center}
\vspace{-1pt}
   \caption{Network reapplication without masks.}
\label{reapply_no_mask}
\end{figure*}

==> fig/figure_reapply_details_multinorm.tex <==
\begin{figure*}
\begin{center}
\captionsetup[subfigure]{font=scriptsize}
%
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in4.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar4.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in31.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar31.png}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in4.png}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar4.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_4.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar4_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_4_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar7.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_7.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar7_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_7_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar10.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_10.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar10_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_10_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_31_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar19.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_19.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_post_31.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar19_random/test_2_post_31.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/content/in31.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_4_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_7_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_10_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_19_inv.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_19_inv.PNG}
\end{subfigure}
\hspace{0.086\linewidth}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_31_inv.PNG}
\end{subfigure}

\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/style/tar31.png}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_4.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_7.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_10.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_2_post_19.PNG}
\end{subfigure}
\begin{subfigure}[b]{0.086\linewidth}
\includegraphics[width =\linewidth, height = 0.6\linewidth]{fig/reapply_multinorm/tar31_random/test_post_31.PNG}
\end{subfigure}
\hspace{0.086\linewidth}

\end{center}
\vspace{-1pt}
   \caption{Network reapplication without masks.}
\label{reapply_multinorm_mask}
\end{figure*}

==> fig/figure_teapot.tex <==
\begin{figure}
\captionsetup[subfigure]{font=tiny}
\begin{center}
\begin{subfigure}{0.19\linewidth}
\begin{overpic}[width=\linewidth]{fig/content/in45.png}
\put(-2,60){\color{white}%
	\frame{\includegraphics[width=0.5\linewidth]{fig/style/tar45.png}}}
\end{overpic}
\caption{Content / Style}
\end{subfigure}
\begin{subfigure}{0.19\linewidth}
\includegraphics[width=\linewidth]{fig/luan/best45_t_1000.png}
\caption{Luan \etal\cite{luan17}}
\end{subfigure}
\begin{subfigure}{0.19\linewidth}
\includegraphics[width=\linewidth]{fig/li/example45.png}
\caption{Li \etal\cite{li2018}}
\end{subfigure}
\begin{subfigure}{0.19\linewidth}
\includegraphics[width=\linewidth]{fig/ours/output45.png}
\caption{Ours}
\end{subfigure}
\begin{subfigure}{0.19\linewidth}
\includegraphics[width=\linewidth]{fig/ours/output45_5l.png}
\caption{Ours modified}
\end{subfigure}
\end{center}
   \caption{Photorealistic texture transfer.}
\label{teapot}
\end{figure}
